Graph-based Anomaly Detection and Description: A Survey

Detecting anomalies in data is a vital task, with numerous high-impact applications in areas such as security, finance, health care, and law enforcement. While numerous techniques have been developed in past years for spotting outliers and anomalies in unstructured collections of multi-dimensional points, with graph data becoming ubiquitous, techniques for structured {\em graph} data have been of focus recently. As objects in graphs have long-range correlations, a suite of novel technology has been developed for anomaly detection in graph data. This survey aims to provide a general, comprehensive, and structured overview of the state-of-the-art methods for anomaly detection in data represented as graphs. As a key contribution, we provide a comprehensive exploration of both data mining and machine learning algorithms for these {\em detection} tasks. we give a general framework for the algorithms categorized under various settings: unsupervised vs. (semi-)supervised approaches, for static vs. dynamic graphs, for attributed vs. plain graphs. We highlight the effectiveness, scalability, generality, and robustness aspects of the methods. What is more, we stress the importance of anomaly {\em attribution} and highlight the major techniques that facilitate digging out the root cause, or the `why', of the detected anomalies for further analysis and sense-making. Finally, we present several real-world applications of graph-based anomaly detection in diverse domains, including financial, auction, computer traffic, and social networks. We conclude our survey with a discussion on open theoretical and practical challenges in the field.

==> outline.tex <==

\begin{itemize}
\item[I.] \textbf{Anomaly detection in static graphs} (Section 2)
		\begin{itemize}
		%\item[(a)] Overview: Outliers in clouds of points \\
						%\begin{itemize}
						%\item[i.] 
		%				Outliers in numerical and categorical data points %; distance-based \citep{aggarwal:2001}, density-based \citep{PapadimitriouKGF03}.
						%\item[ii.] 	
%						Outliers in categorical data points \dan{probably out}%\citep{AkogluCIKM12} 
						%\end{itemize}

		\item[(a)]  Anomalies in plain (unlabeled) graphs
		\item[(b)]  Anomalies in attributed (node-/edge-labeled) graphs
		%Anomaly detection in static \emph{graph} data
%						\begin{itemize}
%						\item[i.]  Anomalies in plain (unlabeled) graphs %\citep{Akoglu2009oddball},\citep{SunQCF05}
%						\item[ii.] Anomalies in attributed (node-/edge-labeled) graphs %\citep{EberleH07},\citep{NobleC03}
%						\end{itemize}
		\end{itemize}
		
\item[II.] \textbf{Anomaly detection in dynamic graphs} (Section 3)
		\begin{itemize}
		
		\item[(a)] Feature-based events
		\item[(b)] Decomposition-based events
		\item[(c)] Community- or clustering-based events
		\item[(d)] Window-based events
		
%		\item[(a)] Overview: Anomaly detection in time series of data points
%						%\begin{itemize}
%						%\item[i.]  
%						
%						Modeling and change detection in time-series data %\citep{ChandolaBK12}
%%						\item[ii.] Change detection in sequence data % \citep{Tsymbal:2004}
%						%\end{itemize}		
%		\item[(b)] Anomaly detection in time series of \emph{graph} data
%						\begin{itemize}
%						\item[i.]  Graph-invariants-based events %\citep{BPincombe05}
%						\item[ii.] Decomposition-based events %Change detection based on graph connectivity %\citep{Akoglu2010army}, \citep{SunFPY07}
%						\item[iii.] Community- or clustering-based events
%						\item[iv.] Window-based events
%						\end{itemize}		
		\end{itemize}
		
\item[III.]  \textbf{Graph-based anomaly description} (Section 4)
		\begin{itemize}
		
			\item[(a)]  Interpretation-friendly graph anomaly detection%attribution, identifying the culprits
			\item[(b)]  Interactive graph querying and sense making
						
						
%		\item[(a)] Theory and Algorithms: %Introduction to relational learning
%						\begin{itemize}
%						\item[i.]  Exploiting graph structure %\citep{SenNBGGE08},\citep{Neville03}
%						\item[ii.] Exploiting graph proximity % \citep{TaskerPK02}, \citep{Getoor+al:SRL07}
%						\item[iii.] Exploiting relational learning
%						\end{itemize}
		
%		 \item[(b)] Real-world Applications: % Relational classification for fraud detection
%						%\begin{itemize}
%						%\item[i.]  
%						
%						Telecommunications fraud, online auction fraud, %\citep{PanditCWF07}
%						accounting fraud risk, \\ securities fraud, review/opinion spam, financial trading fraud, %\citep{AkogluFraud12}
%						%\item[ii.] 
%						%Review/opinion spam, %\citep{McGlohonBASF09},
%						web spam \\ and malware, network intrusion % \citep{NevilleSJKPG05}
%						%\end{itemize}		
		\end{itemize}		

\item[IV.]  \textbf{{Graph}-based anomaly detection in real-world applications} (Section 5)

\begin{tabular}{l  l}
\hspace{-0.15in} (a) Anomalies in telecom networks & \hspace{-0.1cm}     (f) Anomalies in opinion networks \\
\hspace{-0.15in} (b) Anomalies in auction networks & \hspace{-0.1cm}     (g) Anomalies in the Web network \\
\hspace{-0.15in} (c) Anomalies in account networks & \hspace{-0.1cm}     (h) Anomalies in social networks \\
\hspace{-0.15in} (d) Anomalies in security networks & \hspace{-0.1cm}     (i) Anomalies in computer networks \\
\hspace{-0.15in} (e) Anomalies in financial networks & \hspace{-0.1cm}     \\
\end{tabular}
				

\end{itemize}
